Optimizing carrier balance in CsPbBr3 nanocrystal LEDs: The role of alkyl ligands and polar electron transport layers

The study of lead halide perovskite nanocrystal based light-emitting diodes (LEDs) has advanced significantly, with notable improvements in stability and optical properties. However, optimizing charge carrier injection and transport remains a challenge. Efficient electroluminescence requires a balanced transport of both holes and electrons within the emitting material. Here, we investigate cubic CsPbBr\textsubscript{3} nanocrystals passivated with oleylamine and oleic acid, comparing them to ligand-exchanged nanocrystals with didodecyldimethylammonium bromide (DDABr). Nuclear magnetic resonance spectroscopy and transmission electron microscopy confirm successful ligand exchange, revealing reduced ligand coverage in DDABr-treated nanocrystals. Photoelectron spectroscopy, spectroelectrochemistry, and single-carrier devices indicate improved hole injection in DDABr-capped nanocrystals. Density functional theory calculations further reveal the influence of ligand type and coverage on energy levels, with oleic acid introducing localized states in native nanocrystals. Additionally, incorporation of a polar electron transport layer (ETL) enhances LED performance by over an order of magnitude in DDABr-capped nanocrystals, driven by improved charge balance arising from the spontaneous orientation polarization (SOP) of the ETL. These findings highlight the critical role of ligand selection, passivation degree, and charge transport control by the adjacent organic transport layers in optimizing LED efficiency.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
